Multivariate Big Data Analysis for Intrusion Detection: 5 steps from the haystack to the needle

The research literature on cybersecurity incident detection & response is very rich in automatic detection methodologies, in particular those based on the anomaly detection paradigm. However, very little attention has been devoted to the diagnosis ability of the methods, aimed to provide useful information on the causes of a given detected anomaly. This information is of utmost importance for the security team to reduce the time from detection to response. In this paper, we present Multivariate Big Data Analysis (MBDA), a complete intrusion detection approach based on 5 steps to effectively handle massive amounts of disparate data sources. The approach has been designed to deal with the main characteristics of Big Data, that is, the high volume, velocity and variety. The core of the approach is the Multivariate Statistical Network Monitoring (MSNM) technique proposed in a recent paper. Unlike in state of the art machine learning methodologies applied to the intrusion detection problem, when an anomaly is identified in MBDA the output of the system includes the detail of the logs of raw information associated to this anomaly, so that the security team can use this information to elucidate its root causes. MBDA is based in two open software packages available in Github: the MEDA Toolbox and the FCParser. We illustrate our approach with two case studies. The first one demonstrates the application of MBDA to semistructured sources of information, using the data from the VAST 2012 mini challenge 2. This complete case study is supplied in a virtual machine available for download. In the second case study we show the Big Data capabilities of the approach in data collected from a real network with labeled attacks.

==> Sections/relatedPGT.tex <==

IDS paradigms rely on data analysis to determine the ocurrence of potential harmful activities and threats. For that, machine and network related events are usually considered as input observations from which to extract patterns and estimate behaviours \cite{Buczak18}. However, provided the size and complexity of current network systems and the usual high speed of such environments, the amount and variety of data to be processed with detection purposes becomes almost unmanageable.

In this context, Big Data analytics constitutes a major challenge and opportunity for intrusion detection. Big Data is usually characterized and expressed in terms of 4Vs: volume ({\it i.e.}, amount, size, and scale of the data), velocity ({\it i.e.}, speed at which data are generated, and rate at which they must be analyzed), variety ({\it i.e.}, heterogeneity of the data in terms of semantics and sources) and  veracity ({\it i.e.}, reliability of the data in terms of provenance and quality). A fifth V is sometimes included: value ({\it i.e.}, the worth of the data to be analyzed), although some authors defend that it is not inherent to Big Data itself \cite{Heureux17}. Mainly focused on volume, velocity and variety, authors in \cite{Zuech15} present the overall Big Data problem from different technical perspectives: feature selection, data reduction, information fusion and processing techniques. A similar general discussion can be found in \cite{Wang17}, while more specific technical proposals in the field are as follows.  

Regarding feature selection, Huang et {\it al.} explore in \cite{Huang14} a hybrid IDS approach through knowledge discovery from big data using Latent Dirichlet Allocation (LDA). However, no practical detection results in real environments are provided by the authors. Novel feature selection methods, namely, RFFSR (RandomForest-Forward Selection Ranking) and RF-BER (RandomForest-Backward Elimination Ranking) are proposed in \cite{Jarrah14}, but KDD99 dataset is used for evaluation which is outdated as a valid IDS experimentation and far from being considered as a Big Data scenario. The same flawed assessment dataset is considered in \cite{Rachburee17}, where mutual information and chi-square are used as a feature selection technique to reduce a feature set for computation time. 

Rehman et {\it al.} present a review of methods used for big data reduction in \cite{Rehman16}. Some elementary proposals like that in \cite{Meng18} pose to reduce data for wireless intrusion detection in IoT environments by simple traffic sampling, either systematic or random. Authors in \cite{Dahiya18} propose a framework in which two feature reduction algorithms, Canonical Correlation Analysis (CCA) and Linear Discriminant Analysis (LDA), are used for reducing the less important features for fast, efficient and accurate detection of intrusion in the netflow records using Spark. Aimed to reduce dimensionality, Principal Component Analysis (PCA) is recurrently used in the literature. For examle, in \cite{Vasan16} and \cite{Zhang18}. In the last case, the technique of scanning data by rows is applied to introduce a new PCA approach for big data environments, and the KDD99 dataset is used however again for assessment. 

A comprehensive review of data fusion ({\it i.e.,} association, correlation, and combination of data and information from single and multiple sources) techniques for big data network intrusion detection is provided in \cite{Li18}. In addition to present different fusion levels for data, features and decision taking, the authors specify a general fusion framework and describe different evaluation criteria for fusion techniques.

Regarding analysis and processing techniques for big data intrusion detection, several contributions can also be found in the literature. Peng et {\it al.} propose in \cite{Peng18} a clustering method based on Mini Batch Kmeans with PCA (PMBKM). First, the data are preprocessed to digitize the strings and normalize the ranges. Second, the PCA method is used to reduce the data dimensionality to improve clustering efficiency of a mini batch Kmeans algorithm. However, the implementation is not properly assessed, as the  KDD CUP99 dataset is used again for experimentation. A similar situation occurs with \cite{Othman18}, where authors propose an intrusion detection model by using support vector machine (SVM) classifer on Apache Spark Big Data platform.

Additional contributions are provided in \cite{Krotofil15} and \cite{Xie18} in regards with veracity. In the first case, the authors propose an entropy-based anomaly detection system to identify attacks over the veracity of the system, such as data injection. Xie et {\it al.} introduce in \cite{Xie18} Pagoda, a hybrid approach that takes into acount the anomaly degree of a single provenance path as well as the whole provenance path to quickly detect serious compromises on a path. Despite the technical development, the experimentation is flawed again, as very few traces of some network applications are considered to assess the system.

Also related to veracity, a recurrent neural network-based Big Data approach is introduced in \cite{Gulmez18} for cloud intrusion detection. In \cite{Moustafa17}, a Dirichlet mixture model is proposed for lightweight anomaly detection using a lower-upper interquartile range as a decision taking method. %In both cases the UNSW-NB15 dataset is considered for experimentation. 

Based on MSNM \cite{MSNM2015}, we introduce here MBDA (Multivariate Big Data Analysis) as a complete intrusion detection and analysis approach supported on the Big Data functionality of the MEDA Toolbox \cite{Camacho15} to calibrate the anomaly detection model. This makes possible to detect and isolate outliers that may affect the model performance. On the other hand, a new tool named the FCParser (https://github.com/josecamachop/FCParser) has been developed to work in association with MSNM. This tool transforms raw data into analysis features and the other way round, so that we can extend the MSNM diagnosis to the original Big Data stream. This way, security professionals can use MBDA without any knowledge of multivariate analysis, something which was not possible with MSNM. This enhancement is expected to be very effective in reducing the time from detection to response in the face of cybersecurity incidents.   

Moreover, it is important to mention that the proposal will be assessed with adequate Big Data datasets.











